Approximating Petri Net Reachability Along Context-free Traces

We investigate the problem asking whether the intersection of a context-free language (CFL) and a Petri net language (PNL) is empty. Our contribution to solve this long-standing problem which relates, for instance, to the reachability analysis of recursive programs over unbounded data domain, is to identify a class of CFLs called the finite-index CFLs for which the problem is decidable. The k-index approximation of a CFL can be obtained by discarding all the words that cannot be derived within a budget k on the number of occurrences of non-terminals. A finite-index CFL is thus a CFL which coincides with its k-index approximation for some k. We decide whether the intersection of a finite-index CFL and a PNL is empty by reducing it to the reachability problem of Petri nets with weak inhibitor arcs, a class of systems with infinitely many states for which reachability is known to be decidable. Conversely, we show that the reachability problem for a Petri net with weak inhibitor arcs reduces to the emptiness problem of a finite-index CFL intersected with a PNL.

==> part2.tex <==


\subsubsection{Part 2.}


In this section, we  show that it is possible to construct a $\pnw$ $N'$ such that  the problem whether  the call to the procedure  \(\mathit{traverse}(A^{[k]})\)
successfully returns  can be reduced, in polynomial time, to the reachability problem for $N'$ (which is a decidable problem). This implies that the reachability problem for $\pn$ along finite-index $\cfl$ is decidable.

\begin{lemma}
\label{lem2-part2}
Let $\ell \in \set{0,\ldots,k}$, $X^{[\ell]}\in\mathcal{X}^{[k]}$, and
$\mmap,\mmap'\in\multiset{S}$. Then, we can construct a $\pnw$ $N_{X^{[\ell]}}$
such that the proper call \(\mathit{traverse}(X^{[\ell]})\) with 
$\mathbf{M_{\sf i}}[\ell]=\mmap$, $\mathbf{M_{\sf i}}[\ell]=\mmap'$
successfully returns if{}f the multiset $\varnothing$ is
reachable in $N_{X^{[\ell]}}$.
\end{lemma}

The remaining part of this section is devoted to the proof of Lemma
\ref{lem2-part2}.   Notice that we do not give the formal definition of
$N_{X^{[\ell]}}$  but  we provide the description  below together with some
intuitions which allow to reconstruct $N_{X^{[\ell]}}$ easily. 

\begin{proof}
The  $\pnw$
$N_{X^{[\ell]}}$ can be constructed from the code of \(\mathit{traverse}\) as
follows:  

\begin{itemize}
  \item For each variable $Y^{[j]} \in \mathcal{X}^{[k]}$ with $j \leq \ell$, $N_{X^{[\ell]}}$ has  a place $y^{[j]}$. A token in $y^{[j]}$ means that the call \(\mathit{traverse}(Y^{[j]})\) is being simulated. Each of those places contains at most \(1\) token.
  \item For each $p \in \prod^{[k]}$ and  $j \leq \ell$,  $N_{X^{[\ell]}}$ has  a place $p^{[j]}$. A token in $p^{[j]}$ 
    where \(\mathit{head}(p)=X^{[j]}\) for some \(X\in\mathcal{X}\) means that 
    the call \(\mathit{traverse}(X^{[j]})\) picked \(p\) at line~\ref{ln:pick}. Each of those places contains at most \(1\) token.
\item For each place $s $ of $N$ and index  $j \leq \ell$,  $N_{X^{[\ell]}}$ has two places $s_{\sf i}^{[j]}$ and $s_{\sf f}^{[j]}$. The set of places $S_{\sf i}^{[j]}=\{s_{\sf i}^{[j]} \, |\, s \in S\}$ (resp. $S_{\sf f}^{[j]}=\{s_{\sf f}^{[j]} \, |\, s \in S\}$) is used by $N_{X^{[\ell]}}$ to keep the value of the global variable $\mathbf{M_{\sf i}}[j]$ (resp. $\mathbf{M_{\sf f}}[j]$). 

\item For each  index  $j \leq \ell$ and control location (or line number) ${ln}$ of the procedure \(\mathit{traverse}\), $N_{X^{[\ell]}}$ has a place $c_{ln}^{[j]}$. A token in $c_{ln}^{[j]}$ means that the statement at line \(ln\) is next to be simulated. Each of those places contains at most \(1\) token.
\end{itemize}


The initial marking of $N_{X^{[\ell]}}$ puts one token in the place
$x^{[\ell]}$ (\(N_{X^{[\ell]}}\) is going to simulate the call
\(\mathit{traverse}(X^{[\ell]})\)), one token in the place $c^{[\ell]}_1$ (the
simulation starts at line 1), $\mmap(s)$ (resp. $\mmap'(s)$) tokens in the place $s_{\sf
i}^{[\ell]}$ (resp. $s_{\sf f}^{[\ell]}$) for all
$s \in S$ (\(N_{X^{[\ell]}}\) simulates \(\mathit{traverse}(X^{[\ell]})\) for context \(\mathbf{M_{\sf i}}[\ell]=\mmap\) and \(\mathbf{M_{\sf f}}[\ell]=\mmap'\)), and zero token elsewhere in $N_{X^{[\ell]}}$ (the call that \(N_{X^{[\ell]}}\) simulates is proper).


Now,  let us explain how $N_{X^{[\ell]}}$ simulates a proper call
\(\mathit{traverse}(X^{[\ell]})\). To this aim, we proceed by induction on the
index $\ell$.

\medskip %
\noindent %
{\bf Basis.} $\ell=0$.  To simulate  the call \(\mathit{traverse}(X^{[0]})\),
$N_{X^{[0]}}$ proceeds as follows: First, $N_{X^{[0]}}$ moves one token from
the place $c^{[0]}_1$ to $c^{[0]}_3$ since the assert statement at line
\ref{ln:verif} is (vacuously) true. Then, $N_{X^{[0]}}$ checks that there is
one token in the place $x^{[0]}$, chooses (in non-deterministic way)  to  put
one token in the place $p^{[0]}$ such that $\mathit{head}(p) = X^{[0]}$, and
moves one token from the place $c^{[0]}_3$ to $c^{[0]}_6$. This step
simulates that the fact that a proper call \(\mathit{traverse}(X^{[0]})\)
necessarily executes the case of line~\ref{ln:case0}.

Suppose the assert statement of line~\ref{ln:assertbasic} succeeds. In this
case $N_{X^{[0]}}$ faithfully simulates this success if it can empty (using
ad-hoc transitions) every of its places after firing the transition $\sigma$
(if $\sigma \neq \epsilon$ else nothing) on the set of places $S_{\sf
i}^{[0]}$. The only possibility for \(N_{X^{[0]}}\) to empty its places is to
fire \(\sigma\) and reach a marking such that $s_{\sf i}^{[0]}$ and $s_{\sf
f}^{[0]}$ contains an equal number of tokens for every \(s\in S\).

\medskip %
\noindent %
{\bf Step.} $\ell>0$.   Let us describe how any statement executable during the call
\(\mathit{traverse}(X^{[\ell]})\) can be simulated in $N_{X^{[\ell]}}$.   

To simulate the  assert statement at lines  \ref{ln:verif}, \ref{assert1} and
\ref{assert2} (whether $\mathbf{M_{\sf i}}[j]={\mathbf{M_{\sf f}}}[j]=
\varnothing $ \  for all $j<\ell$) of Alg.~\ref{alg:traverse}, $N_{X^{[\ell]}}$
checks if the places associated with $N_{X^{[\ell-1]}}$ are empty.


The simulation of the statement at line \ref{ln:pick} can be done  as follows:
$(1)$ $N_{X^{[\ell]}}$ checks that there is one token in the place
$x^{[\ell]}$, $(2)$ chooses (in non-deterministic way)  to  put one token in
the place $p^{[\ell]}$ such that $\mathit{head}(p) = X^{[\ell]}$, and $(3)$
moves one token from the place $c^{[\ell]}_3$ to the next statement to be
executed by the call \(\mathit{traverse}(X^{[\ell]})\).

The  first case (i.e., statements at lines  \ref{ln:assertbasic} and
\ref{ln:set1})  can be treated  by $N_{X^{[\ell]}}$ similarly to the basic case
${\ell=0}$. 

\(N_{X^{[\ell]}}\) simulates the procedure \(\mathit{transfer\_from\_to}\) (see
Alg.~\ref{alg:transfer}) by iteratively consuming one token from every place
of $\mathit{src}$ and simultaneously producing
one token in every place of $\mathit{tgt}$.  In our case, this step
corresponds to move some tokens from the place $s_{\sf f}^{[\ell]}$ to the
place $s_{\sf f}^{[\ell-1]}$ (see line \ref{transfer}) or from the place
$s_{\sf i}^{[\ell]}$ to the place $s_{\sf i}^{[\ell-1]}$ (see line
\ref{transfer_bis}) for all $s \in S$.

\(N_{X^{[\ell]}}\) simulates the procedure \(\addto\) (see Alg.
\ref{alg:add}) by iteratively adding one token to every place of
$\mathit{src1}$ and $\mathit{src2}$. This step corresponds to add an equal but
arbitrary number of tokens to the places $s_{\sf f}^{[\ell]}$ and  $s_{\sf
i}^{[\ell-1]}$ (see line \ref{add}) or to the places $s_{\sf i}^{[\ell]}$ and
$s_{\sf f}^{[\ell-1]}$ (see line \ref{add_bis}) for all $s \in S$.

Let us see how \(N_{X^{[\ell]}}\) simulates the recursive calls of
lines~\ref{traverse_c} and \ref{call-l-1_bis}. Let us consider how
\(N_{X^{[\ell]}}\) simulates a recursive call, say
\(\mathit{traverse}(Y^{[\ell-1]})\).  $N_{X^{[\ell]}}$ produces one token
$y^{[\ell-1]}$ and $c_1^{[\ell-1]}$ (the initial control location). Then, the
$\pnw$ $N_{Y^{[\ell-1]}}$ (which is a subnet of $N_{X^{[\ell]}}$) starts to
simulate the call \(\mathit{traverse}(Y^{[\ell-1]})\).  While the call
\(\mathit{traverse}(Y^{[\ell-1]})\) is being simulated, the only transitions of
\(N_{X^{[\ell]}}\) that are firing are those of \(N_{Y^{[\ell-1]}}\).
$N_{X^{[\ell]}}$ can resume the simulation of the caller
\(\mathit{traverse}(X^{[\ell]})\) only when all the places of the callee (i.e.
the places of $N_{Y^{[\ell-1]}}$) are empty. This also simulates the assert
statements of lines~\ref{assert1} and \ref{assert2}.


Finally, \(N_{X^{[\ell]}}\) simulates the tail recursive calls of the form
\(\mathit{traverse}(Y^{[\ell]})\) (see line \ref{traverse_b} and line
\ref{traverse_c_bis}) as follows: First, $N_{X^{[\ell]}}$ consumes a token in
the place associated with the current control location, a token in the place
associated with the current input variable $x^{[\ell]}$, and a token in the place
associated with the current executed production $p^{[\ell]}$; and it produces
one token in the place $c_1^{[\ell]}$ associated with the initial control
location, and one token in the place $y^{[\ell]}$ associated with the new initial
input variable.

Observe that the inductive definition of $N_{X^{[\ell]}}$ shows the zero tests
of the $\pnw$ respect the condition imposed by Reinhardt and given at \eqref{eq:reinhardt}.

For the if direction of the proof let us consider the contraposition: if
\(\varnothing\) is unreachable in \(N_{X^{[\ell]}}\) then the proper call
\(\mathit{traverse}(X^{[\ell]})\) does not successfully return.
Let us give the intuition of the proof. Unreachability of \(\varnothing\) means
that along every execution of \(N_{X^{[\ell]}}\), there exists a subset of
places which eventually always contains tokens. Actually from the structure of
\(N_{X^{[\ell]}}\) it can be shown that along every execution, there exists
\(j\leq \ell\) such that \(S_{\sf i}^{[j]}\cup S_{\sf f}^{[j]}\) never gets empty. 
This means that the assert of line~\ref{ln:assertbasic} fails, hence
that a proper call to \(\mathit{traverse}\) does not return successfully,
and finally that no matter how you resolve non determinism in
Alg.~\ref{alg:traverse} the call \(\mathit{traverse}(X^{[\ell]})\) does not successfully
return.\qed

\end{proof}
%
%
It follows from Lemma  \ref{lem1}, \ref{lem:alg_equiv} and \ref{lem2-part2} that:
%
\begin{corollary}
The reachability problem for
\(\pn\) along finite-index \(\cfl\)  can be reduced to the reachability problem for \(\pnw\). 
\end{corollary}

